Using Enriched Category Theory to Construct the Nearest Neighbour Classification Algorithm

This paper is the first to construct and motivate a Machine Learning algorithm solely with Enriched Category Theory, supplementing evidence that Category Theory can provide valuable insights into the construction and explainability of Machine Learning algorithms. It is shown that a series of reasonable assumptions about a dataset lead to the construction of the Nearest Neighbours Algorithm. This construction is produced as an extension of the original dataset using profunctors in the category of Lawvere metric spaces, leading to a definition of an Enriched Nearest Neighbours Algorithm, which, consequently, also produces an enriched form of the Voronoi diagram. Further investigation of the generalisations this construction induces demonstrates how the $k$ Nearest Neighbours Algorithm may also be produced. Moreover, how the new construction allows metrics on the classification labels to inform the outputs of the Enriched Nearest Neighbour Algorithm: Enabling soft classification boundaries and dependent classifications. This paper is intended to be accessible without any knowledge of Category Theory.

==> sections/future_work.tex <==
\section{Future Work}

Given the diversity of Machine Learning algorithms and the natural generalising power of Enriched Category Theory, there are numerous avenues to explore for future extensions of this work.

The construction of the \textit{NNA} in section \ref{section:Construction} does not require any specific properties of Cost-enriched categories to define. This naturally leads to a candidate definition of the V-enriched Nearest Neighbours Algorithm (\textit{V-NNA}).
\begin{small}
\begin{align}
\textit{V-NNA}&: X \nrightarrow Y\\
\textit{V-NNA}&(y, x) := V((\mathbf{1}_{NY} \circ F^*)(y, x),\ (T_*\circ F^*)(y, x)) 
\end{align}
\end{small}

The question arises as to whether this definition has valuable properties in other bases of enrichment. Though the previous section interpreted the hom-object of the base of enrichment in its Bool-enriched form for the sake of clarity, future works would benefit from considering the self-enriched form of the hom-object and, in the case of the Cost-NNA, interpreting the hom-object with truncated subtraction rather than an inequality.
\begin{small}
\begin{align}
\textit{Cost-NNA}&: X \nrightarrow Y\\
\textit{Cost-NNA}&(y, x) = \ (T_*\circ F^*)(y, x)\ \dot{-}\ (\mathbf{1}_{NY} \circ F^*)(y, x) 
\end{align}
\end{small}

Researchers who are not interested in Machine Learning would possibly consider the Voronoi diagram as a more exciting outcome of the \textit{V-NNA}. By assigning each index a separate class, the \textit{NNA} partitions the metric space dependent on each point. In this instance, the partitions generated in other bases of enrichment may prove interesting.

The generalisation of the \textit{NNA} to the \textit{$k$-NNA} shows how the latter can be expressed in terms of the former using the flexible language of profunctor composition. This relationship is not clear in other presentations. Further investigation of how profunctor composition can be used to express machine learning algorithms may lead to deeper insights. Beyond this, the increased flexibility of the enriched \textit{NNA} in allowing $Y$ to take on a variety of metrics requires practical verification to demonstrate its utility on real-world datasets.
